Domain Reduction Strategy for Non Line of Sight Imaging

This paper presents a novel optimization-based method for non-line-of-sight (NLOS) imaging that aims to reconstruct hidden scenes under general setups with significantly reduced reconstruction time. In NLOS imaging, the visible surfaces of the target objects are notably sparse. To mitigate unnecessary computations arising from empty regions, we design our method to render the transients through partial propagations from a continuously sampled set of points from the hidden space. Our method is capable of accurately and efficiently modeling the view-dependent reflectance using surface normals, which enables us to obtain surface geometry as well as albedo. In this pipeline, we propose a novel domain reduction strategy to eliminate superfluous computations in empty regions. During the optimization process, our domain reduction procedure periodically prunes the empty regions from our sampling domain in a coarse-to-fine manner, leading to substantial improvement in efficiency. We demonstrate the effectiveness of our method in various NLOS scenarios with sparse scanning patterns. Experiments conducted on both synthetic and real-world data support the efficacy in general NLOS scenarios, and the improved efficiency of our method compared to the previous optimization-based solutions. Our code is available at https://github.com/hyunbo9/domain-reduction-strategy.

==> Main/Partials/table_memory.tex <==
% \hfill
% \begin{table}[t]

% \begin{adjustbox}{valign=t}
% \begin{minipage}{0.4\linewidth}

% \setlength{\tabcolsep}{3pt}
% \centering
% \small
% \caption{Ablation results on the domain reduction. 'Red.' denotes the domain reduction and 'C2F' denotes the coarse-to-fine strategy. We report elapsed time (seconds) of the optimization and the ratio of remaining domain in the parentheses at each step.}

% \begin{tabular}{cc|c}
% \toprule
%  & 500 iter & 1000 iter \\
% \midrule
%  539 s & 539 s & 1087 s \\
%  539 s & 103 s (4\%) & 134 s (4\%) \\
%  539 s & 27 s (3\%) & 54 s (3\%) \\
% \bottomrule
% \end{tabular}

% \label{table:ablation_reduction}
% \vspace{-10pt}

% \end{minipage}
% \end{adjustbox}
% \end{table}


==> Main/Partials/table_total.tex <==
\begin{table}[t]

\begin{adjustbox}{valign=t}
\begin{minipage}{0.4\linewidth}

\setlength{\tabcolsep}{3pt}
\centering
\small
\caption{Ablation results on the domain reduction. 'Red.' denotes the domain reduction and 'C2F' denotes the coarse-to-fine strategy. We report elapsed time (seconds) of the optimization and the ratio of remaining domain in the parentheses at each step.}

\begin{tabular}{cc|cccc|c}
\toprule
Red. & C2F & 100 iter & 500 iter & 1000 iter \\
\midrule
 &  & 109  & 539 s & 1087 s \\
\checkmark & & 67 s (11\%) & 103 s (4\%) & 134 s (4\%) \\
\checkmark & \checkmark & 4 s (15\%) & 27 s (3\%) & 54 s (3\%) \\
\bottomrule
\end{tabular}

\label{table:memory}
\vspace{-10pt}

\end{minipage}
\end{adjustbox}
\end{table}


==> Rebuttal/Partials/figure_256_bunny.tex <==
\begin{figure}[t]
\vspace{-5pt}
\centering
\includegraphics[trim={0 0 0 0}, width=1\linewidth]{Rebuttal/Assets/rebuttal_256.pdf}
\vspace{-20pt}
\caption{Results on $256 \times 256$ transients of ZNLOS Bunny.}
\vspace{-5pt}
\label{fig:rebuttal_256}
\end{figure}

==> Rebuttal/Partials/figure_sparse_meas.tex <==
\begin{figure}[t]
\centering
\vspace{-5pt}
\includegraphics[trim={0 0 0 0}, width=1\linewidth]{Rebuttal/Assets/rebuttal_sparse.pdf}
\vspace{-20pt}
\caption{
Results on $128\times128$ upsampled transients.
\textbf{(top)} Results on $32 \times 32$ samplings upsampled with a linear interpolation.
\textbf{(bottom)} Results on $16\times16$ samplings, upsampled by filling unsampled pixels with zero.
FFT-based methods produce unfavorable results with artifacts regardless of the upsampling techniques.
}
\vspace{-15pt}
\label{fig:rebuttal_sparse}
\end{figure}

==> Rebuttal/Partials/table_runtime.tex <==
\begin{table}[]
\setlength{\tabcolsep}{4pt}
\centering
\footnotesize
\begin{tabular}{c|ccccc}
\toprule
Time & LCT & FK & NeTF & Ours (w/o reduction) & Ours \\
%\midrule
%complexity & $O(N^3 logN)$ & $O(N^3 logN)$ & $O(N^3)$ & $O(c \cdot N^3)$ \\
\midrule
Recon. & 0.12 s & 0.10 s & $>$ 1 h & 1087 s & 54 s  \\
Scan & 46 m & 46 m & 2 m 49 s & 2 m 49 s & 2 m 49 s \\
\bottomrule
\end{tabular}
\vspace{-5pt}
\caption{
Reconstruction time (Recon.) and scanning time (Scan) required for producing $128\times128$ results of Bunny in high-quality.
% While FFT-based methods (LCT, FK) offer faster reconstruction time, they require time-consuming dense scanning procedures.
We use GPU versions [5] of LCT and FK to report their runtime.
}
\vspace{-12pt}
\label{table:rebuttal_runtime}
\end{table}

==> Rebuttal/rebuttal.tex <==
\input{Rebuttal/Partials/figure_sparse_meas}

We appreciate all reviewers for their valuable comments. We will thoroughly incorporate all feedback in the revision.

\textblock{(\revone, \revthree) Sparse measurements.}
Reconstructing high-resolution volumes from undersampled sparse measurements is an ill-posed problem.
Previous FFT-based methods require measurements to have the same resolution with the target volumes.
One may apply interpolation techniques to upsample the measurements to the desired resolution, as commented by R3.
However, this inevitably introduces approximation errors between upsampled and actual measurements (see \Fref{fig:rebuttal_sparse}, and the supplement Fig. 9).
Therefore, solutions of all methods exhibit approximation errors, which become larger as scanning patterns become sparser.
Optimization-based methods are capable of finding solutions with minimal errors through iterative minimization procedures.
This is further highlighted in results on $16 \times 16$ transients, which are presented in the bottom of \Fref{fig:rebuttal_sparse}.

\textblock{(\revone) Results on $256\times256$ measurements.}
We deliver the results on $256 \times 256$ measurements in \Fref{fig:rebuttal_256}. 
All methods produce compelling results with sufficient scan points.
We thank for the comment and will update them in the revision.

\textblock{(\revone) Computation time comparison.}
We deliver the runtime and scanning time comparisons with existing methods in \Tref{table:rebuttal_runtime}.
While FFT-based methods exhibit fastest reconstruction time, they require exhaustive dense scanning, which is time consuming and becomes another bottleneck.

\textblock{(\revtwo) Captions and overview for clarity.}
We sincerely appreciate the suggestions for improving clarity of our work.
We will update captions to be more comprehensive, and add an overview of the method to provide better understandings.

\textblock{(\revtwo) Test scenes.}
While our experiments follow typical NLOS setups for test scenes, as mentioned by R2, we also believe that analysis with more complex scenes could provide better insights.
We appreciate the insightful comment, and we will add more discussion in the revision.


\textblock{(\revtwo) Related work.}
We thank for suggesting important related work in NLOS imaging, which could make our work more comprehensive.
We will include reviews of the suggested work with detailed descriptions in the revision.

\textblock{(\revthree) Optimization and FFT-based methods.}
We would like to first demonstrate that the goal of this paper is not to achieve the fastest reconstruction speed.
Instead, our goal is to identify efficiency bottlenecks inherent in previous optimization-based methods, particularly stemming from computations related to empty regions.
Consequently, our domain reduction achieves substantial efficiency improvement (see Table 2 of the main paper), while inheriting the general applicability of the optimization framework.

While FFT-based methods benefit from computational efficiency based on the convolutional theorem or Stolt's method, several assumptions have to be made to achieve this, \eg dense scanning points, planar relay walls, or ignoring surface normals.
Some approximations could relax certain assumptions, but at the cost of sacrificing performance.
In contrast, optimization-based methods are more generally applicable to various scenarios, with the potential for continuous modeling, joint optimization of noise parameters, arbitrary BRDF [35], and sparse samplings [24].
Our domain reduction effectively addresses computational burdens of optimization frameworks, paving the way to unleash their full potential.
We hope the reviewer to consider the advantages of optimizations over FFT, and re-evaluate our method in the context of the optimization framework.

We acknowledge that integrating the efficiency of FFT with optimization-based solutions, and possibly with our domain reduction, could yield significant improvements.
Although it is not currently available while preserving general applicability (see Table 4), we believe that this integration will be an interesting avenue for future work.
We will update a detailed discussion on this subject in the revision.

\input{Rebuttal/Partials/figure_256_bunny}
\input{Rebuttal/Partials/table_runtime}
% Advantages of optimization over FFT-based methods -> continuous, 
% our method significantly reduces computations of the typical optimization procedures
% we acknowledge and believe that combining computational efficiency of FFT with the general applicability of optimization could be a very interesting future direction.
% In this manner, we also belive that integreating the proposed domain reduction techniques to such future work could enable a wide range of applications~~ or unleash potentials of NLOS imaging?
